Context-theoretic Semantics for Natural Language: an Algebraic Framework

Techniques in which words are represented as vectors have proved useful in many applications in computational linguistics, however there is currently no general semantic formalism for representing meaning in terms of vectors. We present a framework for natural language semantics in which words, phrases and sentences are all represented as vectors, based on a theoretical analysis which assumes that meaning is determined by context. In the theoretical analysis, we define a corpus model as a mathematical abstraction of a text corpus. The meaning of a string of words is assumed to be a vector representing the contexts it occurs in in the corpus model. Based on this assumption, we can show that the vector representations of words can be considered as elements of an algebra over a field. We note that in applications of vector spaces to representing meanings of words there is an underlying lattice structure; we interpret the partial ordering of the lattice as describing entailment between meanings. We also define the context-theoretic probability of a string, and, based on this and the lattice structure, a degree of entailment between strings. Together these properties form guidelines as to how to construct semantic representations within the framework. A context theory is an implementation of the framework; in an implementation strings are represented as vectors with the properties deduced from the theoretical analysis. We show how to incorporate logical semantics into context theories; this enables us to represent statistical information about uncertainty by taking weighted sums of individual representations. We also use the framework to analyse approaches to the task of recognising textual entailment, to ontological representations of meaning and to representing syntactic structure. For the latter, we give new algebraic descriptions of link grammar.

==> commands.tex <==
 
 
\font\cmbig=cmr7 at 74pt
 
 \newcommand{\dropcap}[1]{
 \setbox1=\hbox{\cmbig #1}
\dimen1=\wd1
\dimen2=\ht1
\box1\nointerlineskip
\advance\dimen2 by 1.5pt
\vskip-\dimen2
\advance\dimen1 by -1pt
\hangindent=\dimen1 \hangafter=-4\noindent
}

%\newcommand{\qu}[1]{{\fontfamily{cmr}\fontseries{s}\fontshape{it}\selectfont #1}}
%\newcommand{\qu}[1]{{\cmbig #1}}

==> discussion.tex <==

\subsection{Discussion}

It is our belief that the recent developments in statistical techniques in computational linguistics require an accompanying development in our ideas of what meaning really is. Our idea of meaning is still connected to representations with their foundations in logic, and it is hard to imagine such representations capturing the subtleties of meaning that can be represented using the vector space representations acquired automatically.

What we propose then, is a theory of meaning that incorporates a vector space nature. Such a theory would be in better agreement with modern techniques in computational linguistics, and allow the more ``fine-grained'' descriptions of meaning that accompany them in vector representations.

The theory of meaning we propose has its foundations in the philosophy of Wittgenstein, who said ``Meaning just \emph{is} use'', and Firth, who said ``You shall know a word  by the company it keeps''. That is, the meaning of a sequence of symbols should be determined merely by looking at how they are used, or where they occur in a large amount of text.

The controversial part of what we propose is that meaning should be attached \emph{purely to context} without any assumed reference to the real world. It should be noted that this concept of meaning is quite different to our normal notion of meaning. An example that was proposed to me as an objection to such a definition of meaning is that we know that a \emph{man} is a \emph{human being} and a \emph{human being} is a \emph{mammal}. However, looking at the contexts that these words occur in, we would not expect significant overlap, for example, between the contexts that the word ``man'' and ``mammal'' occur in. There might be some overlap, but arguably not enough to demonstrate that a \emph{man} is a \emph{mammal}, that is that \emph{man} has all the properties of \emph{mammal}. We have to be able to accept, in our proposed definition of meaning that \emph{according to the definition} a man isn't a mammal! This is a consequence of the fact that we do not require our definition of meaning to be connected in any way to the real world, hence we call this view of meaning context-theoretic, as opposed to model-theoretic models of meaning.
%To separate this view of meaning from theories of meaning intended to represent the real world, we call the new interpretation of meaning \emph{context semantics}.\footnote{The term ``context semantics'' has already been used in the context of program analysis, as a less mathematical version of Girard's \emph{Geometry of Interaction} \citep[see for example][]{Girard:95}. Interestingly, the Geometry of Interaction makes use of Hilbert spaces and C* algebras for entirely different reasons to our own use of vector spaces. The use of the word ``context'' here is not related to our use of the term, so we think that no ambiguity will arise.} We may thus talk about the context semantics of a set of terms, in which it is not true that a \emph{man} is a \emph{mammal}, and their \emph{model-theoretic} semantics, in which this is true, as meanings are intended to be connected to a model of the real world.

Context-theoretic semantics places emphasis on the words themselves, and ignores the fact that words may represent concepts. This emphasis on context coincides with the modern use of statistical techniques in computational linguistics which have proved so effective in many applications. Whilst context-theoretic semantics may be dissatisfying from the perspective of some of our intuitive notions of meaning (a man is not a mammal), from a practical perspective context-theoretic semantics has the potential to successfully describe useful relationships in meaning. It is not often that it is practically \emph{useful} to know that a man is a mammal --- and the evidence from statistical techniques seem to show that the useful relationships very often \emph{are} those that are determined by context.

Of course this is not true in every situation; the context-theoretic approach may not be useful for many applications. It seems likely from what we have found that context-theoretic semantics would be good in situations where a limited form of reasoning is required, but in a ``fuzzy'' manner; and may be of limited use in situations which require complex reasoning and inference.

%\subsection{Predictions}
 
The framework makes several predictions about the nature of meaning, which, while they do not place severe limitations on the capabilities of the context-theoretic representation, do point in the direction of certain representations which are more suited to the context theoretic approach. One example is that the framework requires that meaning is \emph{associative}: if $a$, $b$ and $c$ are the representations of natural language expressions, then the product of $(ab)$ with $c$ is the same as the product of $a$ with $(bc)$; we believe this is a natural consequence of accepting that meaning is determined by context. However this would seem to limit the capabilities of the representation
 
% \section{A new philosophy of meaning}


 \section{Summary}
 

==> fruit-bnc.tex <==
\minipage{12cm}{
\begin{verbatim}
end some medicine for her, but she will need fruit and  milk, and some other special things that
our own. Here we give you ideas for foliage, fruit and  various festive trimmings that you can i
part II). However, other strategies can bear fruit  and are described under three sections which
       supper Ñ tomatoes, potato chips, dried fruit and cake. And  they drank water out of tea-cu
erent days, as  the East Berliners queue for fruit and cheap stereos, a Turkish  beggar sleeps i
dening; and  Pests -- how to control them on fruit and vegetables. Both are  produced by the Hen
me,"Silver Queen" is male so will never bear fruit    At the opposite end of the prickliness sca
 lifted away    Like an orange lifted from a fruit-bowl    And darkness, blacker    Than an oil-
ed in your  wreath. Christmas ribbon and wax fruit can be added for colour.  Essentials are scis
e you need to start developing your very own fruit  collection    KEEPING OUT THE COLD    Need e
ly with Jeyes fluid    THE KITCHEN GARDEN    FRUIT    Cut out cankers on fruit trees, except tho
wn and watered    AUTUMN HUES    Foliage and fruit enrich the autumn garden, whether glowing  th
- have forgotten  the maxim: " tel arbre tel fruit ". If I were  willing  to  unstitch the past 
 of three children of Alfred Roger Ackerley, fruit importer  of London, and his mistress, Janett
rful didactic spirit, much that was to  bear fruit in his years as a mature artist. Although thi
e all made with natural vegetable, plant and fruit ingredients  such as chamomile, kukai nut and
ack in the soup.    He re-visits the Copella fruit juice farm in Suffolk, the  business he told 
rategic relationship" with Lotus, the first  fruit of which is a mail gateway between Office and
, choose your plants  carefully to enjoy the fruit of your labour all year round.    PLACES TO V
 and I love chips.  Otherwise I'll nibble on fruit or something to convince myself  that I'm eat
 tone and felt the  softness and warmth of a fruit ripening against a wall? If she  had she migh
ol place to set. Calories per  slice: 395    Fruit Scones with cinnamon Butter    (makes 12)    
ought me water. Another monster gave me some fruit  to eat. A few monsters lay against my body a
ney fungus.    Cut out diseased wood on most fruit trees    VEGETABLES    Continue winter diggin
age and chafing.    Remove old, unproductive fruit trees by cutting them down to  shoulder heigh
ITCHEN GARDEN    FRUIT    Cut out cankers on fruit trees, except those on peaches, plums  and ch
ps  remain, then stir in the sugar and dried fruit. Using a round-  ended knife, stir in the mil
 of a homeland, well others dream too,    De fruit was forbidden an now yu can't chew,    How ca
onnoisseurs. We take a bite from an unusual  fruit. We come away neither nourished nor ravished,
\end{verbatim}
}

==> graphs_config.tex <==
% Local configuration for version 1.53 of graphs.sty. Frank Drewes, 16.11 2003

% The \special macro below must contain the path under which the file
% graphs.header can be found in you local installation. Please modify it
% accordingly.

\special{header=graphs.header}


==> graphs_ps.tex <==
% `special' commands for version 1.53 of graphs.sty. Frank Drewes, 16/11 2003

\def\ps@s{ }
\def\ps@convertnum#1{
	#1 \number\unitlength\ps@s mul 65536 div 72.27 div 72 mul
}

%-----------------------------------------------------------------------------%


\def\ps@rectangle[#1,#2]{% width, height
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		[ \g@ncolour\ps@s\g@ncolourmod ]\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		\iffillednodes true \else false\fi\ps@s
		psrectangle}}

%-----------------------------------------------------------------------------%

\def\ps@circle[#1]{% diameter
\special{"	\ps@convertnum{#1}
		[ \g@ncolour\ps@s\g@ncolourmod ]\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		\iffillednodes true \else false\fi\ps@s
		pscircle}}

%-----------------------------------------------------------------------------%

\def\ps@line(#1,#2){% end x, end y
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\g@ldash\ps@s
		psline}}

%-----------------------------------------------------------------------------%

\def\ps@loopA(#1,#2)(#3,#4){% from (#1,#2) to (#3,#4)
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{#4}
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		psloop}}

%-----------------------------------------------------------------------------%

\def\ps@loopB#1(#2,#3){% angle #1, axis (#2,#3)
\special{"	#1
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		psloopbyangle
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		psloop}}
		
%-----------------------------------------------------------------------------%

\def\ps@looparrowonrectangleA(#1,#2)(#3,#4)[#5,#6]{% 
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{#4}
		\ps@convertnum{#5}
		\ps@convertnum{#6}
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		pslooparrowonrectangle}}

%-----------------------------------------------------------------------------%

\def\ps@looparrowoncircleA(#1,#2)(#3,#4)[#5]{% 
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{#4}
		\ps@convertnum{#5}
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		pslooparrowoncircle}}

%-----------------------------------------------------------------------------%

\def\ps@looparrowonrectangleB#1(#2,#3)[#4,#5]{% 
\special{"	#1
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		psloopbyangle
		\ps@convertnum{#4}
		\ps@convertnum{#5}
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		pslooparrowonrectangle}}

%-----------------------------------------------------------------------------%

\def\ps@looparrowoncircleB#1(#2,#3)[#4]{% 
\special{"	#1
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		psloopbyangle
		\ps@convertnum{#4}
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		pslooparrowoncircle}}

%-----------------------------------------------------------------------------%

\def\ps@deletebox(#1,#2){% width, height in scaled points
\special{"	#1 65536 div
		#2 65536 div
		psdeletebox}}

%-----------------------------------------------------------------------------%

\def\ps@arrowonrectangle(#1,#2) [#3,#4]{% x, y, width, height
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{#4}
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		psarrowonrectangle}}

%-----------------------------------------------------------------------------%

\def\ps@arrowoncircle(#1,#2) [#3]{% x, y, diameter of circle
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		psarrowoncircle}}

%-----------------------------------------------------------------------------%

\def\ps@path(#1,#2)#3{% start coordinates, (xi,yi[,di]) ...
	\def\extractvalues(##1)##2;{%
	  \ifx\endmarker##1\else%
	    \extractvalues##2;\extractvals(##1,0,)%
	  \fi}%
	\def\extractvals(##1,##2,##3,##4){%
	  \ps@convertnum{##1}%
	  \ps@convertnum{##2}%
	  ##3%
	}%
	\special{" mark \extractvalues#3(\endmarker);
			\ps@convertnum{#1}
			\ps@convertnum{#2}
			\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
			[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
			\g@ldash\ps@s
			[ \g@fcolour\ps@s\g@fcolourmod ]\ps@s
			\iffilledareas true \else false\fi\ps@s pspath}}

%-----------------------------------------------------------------------------%

\def\ps@curve#1#2{% base length, (x1,y1,ang1[factor1]) ...
	\def\extractvalues(##1(##2;##3{%
	  \ifx\endmarker##1\else%
	    \extractvalues(##2;{##3}\extractvals(##1[##3,##3];%
	  \fi}%
	\def\extractvals(##1,##2,##3)[##4,##5]##6;{%
	  ##5\ps@s
	  ##4\ps@s
	  ##3\ps@s
	  \ps@convertnum{##2}%
	  \ps@convertnum{##1}%
	}%
	\special{" mark \extractvalues#2(\endmarker(;{#1}
			\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
			[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
			\g@ldash\ps@s
			[ \g@fcolour\ps@s\g@fcolourmod ]\ps@s
			\iffilledareas true \else false\fi\ps@s pscurve}}

%-----------------------------------------------------------------------------%

\def\ps@bubble#1#2{% length factor, (x1,y1) ...
	\def\extractvalues(##1)##2;{%
	  \ifx\endmarker##1\else%
	    \extractvalues##2;\extractvals(##1)%
	  \fi}%
	\def\extractvals(##1,##2){%
	  \ps@convertnum{##2}%
	  \ps@convertnum{##1}%
	}%
	\special{" mark \extractvalues#2(\endmarker);
			#1\ps@s
			\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
			[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
			\g@ldash\ps@s
			[ \g@fcolour\ps@s\g@fcolourmod ]\ps@s
			\iffilledareas true \else false\fi\ps@s psbubble}}

%-----------------------------------------------------------------------------%

\def\ps@dirbowoncircle(#1,#2)(#3,#4,#5)[#6]{% (x1,x2) (y1,y2,d), radius
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{#4}
		#5\ps@s
		\ps@convertnum{#6}
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\g@ldash\ps@s
		psdirbowoncircle}}

%-----------------------------------------------------------------------------%

\def\ps@dirbowonrectangle(#1,#2)(#3,#4,#5)[#6,#7]{% (x1,x2) (y1,y2,d),
                                                  % xsize, ysize
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{#4}
		#5\ps@s
		\ps@convertnum{#6}
		\ps@convertnum{#7}
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\g@ldash\ps@s
		psdirbowonrectangle}}

%-----------------------------------------------------------------------------%



==> index-extras.idx.tex <==
\indexentry{model-theoretic semantics|see{logical semantics}}{1}
\indexentry{textual entailment|see{entailment}}{1}
\indexentry{lattice!vector|see{vector lattice}}{1}
\indexentry{AL space|see{abstract Lebesgue space}}{1}
\indexentry{probability!context theoretic|see{context theoretic probability}}{1}
\indexentry{LSA|see{latent semantic analysis}}{1}
\indexentry{is-a relation|see{hypernymy}}{1}
\indexentry{distance measures!distributional|see{distributional similarity}}{1}
\indexentry{Riesz space|see{vector lattice}}{1}

==> matrices.tex <==
%Created by jPicEdt 1.x
%Standard LaTeX format (emulated lines)
%Fri Jun 16 08:20:42 BST 2006
\unitlength 1mm
\begin{picture}(120.00,30.00)(0,0)

\linethickness{0.15mm}
%Rectangle(32.00,7.50)(56.00,30.00)  
\put(32.00,7.50){\line(1,0){24.00}}
\put(32.00,7.50){\line(0,1){22.50}}
\put(56.00,7.50){\line(0,1){22.50}}
\put(32.00,30.00){\line(1,0){24.00}}
%End Rectangle

\linethickness{0.15mm}
%Rectangle(0.00,0.00)(24.00,30.00)  
\put(0.00,0.00){\line(1,0){24.00}}
\put(0.00,0.00){\line(0,1){30.00}}
\put(24.00,0.00){\line(0,1){30.00}}
\put(0.00,30.00){\line(1,0){24.00}}
%End Rectangle

\linethickness{0.15mm}
%Rectangle(64.00,7.50)(120.00,30.00)  
\put(64.00,7.50){\line(1,0){56.00}}
\put(64.00,7.50){\line(0,1){22.50}}
\put(120.00,7.50){\line(0,1){22.50}}
\put(64.00,30.00){\line(1,0){56.00}}
%End Rectangle

\linethickness{0.15mm}
%Rectangle(32.00,15.00)(48.00,30.00)  
\put(32.00,15.00){\line(1,0){16.00}}
\put(32.00,15.00){\line(0,1){15.00}}
\put(48.00,15.00){\line(0,1){15.00}}
\put(32.00,30.00){\line(1,0){16.00}}
%End Rectangle

\linethickness{0.15mm}
%Rectangle(0.00,0.00)(16.00,30.00)  
\put(0.00,0.00){\line(1,0){16.00}}
\put(0.00,0.00){\line(0,1){30.00}}
\put(16.00,0.00){\line(0,1){30.00}}
\put(0.00,30.00){\line(1,0){16.00}}
%End Rectangle

\linethickness{0.15mm}
%Rectangle(64.00,15.00)(120.00,30.00)  
\put(64.00,15.00){\line(1,0){56.00}}
\put(64.00,15.00){\line(0,1){15.00}}
\put(120.00,15.00){\line(0,1){15.00}}
\put(64.00,30.00){\line(1,0){56.00}}
%End Rectangle

\end{picture}


==> orange-fruit.tex <==
jPicEdt default formatter factory [pending]Mon Jan 22 14:11:29 GMT 2007
[Rectangle@ecb06:
	attrib_set={}
	pts[0]=(0.0,0.0) pts[1]=(2.5,10.0) 
][Rectangle@331ce6:
	attrib_set={}
	pts[0]=(5.0,0.0) pts[1]=(7.5,5.0) 
][Rectangle@ae48dc:
	attrib_set={}
	pts[0]=(15.0,0.0) pts[1]=(17.5,35.0) 
][Rectangle@317d82:
	attrib_set={}
	pts[0]=(25.0,0.0) pts[1]=(27.5,15.0) 
][Rectangle@270aef:
	attrib_set={}
	pts[0]=(40.0,0.0) pts[1]=(42.5,5.0) 
][Rectangle@3f02bd:
	attrib_set={}
	pts[0]=(45.0,0.0) pts[1]=(47.5,15.0) 
][Rectangle@ccec5f:
	attrib_set={}
	pts[0]=(50.0,0.0) pts[1]=(52.5,20.0) 
][Rectangle@b289cd:
	attrib_set={}
	pts[0]=(55.0,0.0) pts[1]=(57.5,15.0) 
][Rectangle@751a9b:
	attrib_set={}
	pts[0]=(60.0,0.0) pts[1]=(62.5,25.0) 
][Rectangle@25e068:
	attrib_set={}
	pts[0]=(65.0,0.0) pts[1]=(67.5,15.0) 
][Polygon@afceff:
	attrib_set={}
	pts[0]=(-2.5,0.0) pts[1]=(30.0,0.0) 
] open[Polygon@3ed81c:
	attrib_set={}
	pts[0]=(37.5,0.0) pts[1]=(72.5,0.0) 
] open
Not parsed commands :




==> pentagon.tex <==
%%Created by jPicEdt 1.4: mixed JPIC-XML/LaTeX format
%%Tue Apr 13 16:39:18 BST 2004
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic width="30.62" height="35.62">
%<multicurve points="(3.75,23.75);(3.75,23.75);(13.75,33.75);(13.75,33.75)"
%	 stroke-width="0.3" stroke-color="#000000"
%	 fill-style="none"
%	 />
%<multicurve points="(3.75,23.75);(3.75,23.75);(3.75,13.75);(3.75,13.75)"
%	 stroke-width="0.3" stroke-color="#000000"
%	 fill-style="none"
%	 />
%<multicurve points="(3.75,13.75);(3.75,13.75);(13.75,3.75);(13.75,3.75)"
%	 stroke-width="0.3" stroke-color="#000000"
%	 fill-style="none"
%	 />
%<multicurve points="(13.75,3.75);(13.75,3.75);(28.75,18.75);(28.75,18.75)"
%	 stroke-width="0.3" stroke-color="#000000"
%	 fill-style="none"
%	 />
%<multicurve points="(28.75,18.75);(28.75,18.75);(13.75,33.75);(13.75,33.75)"
%	 stroke-width="0.3" stroke-color="#000000"
%	 fill-style="none"
%	 />
%<ellipse p1="(11.88,35.62)" p2="(15.62,35.62)" p3="(15.62,31.88)" angle-start="0" angle-end="0" closure="open"
%	 stroke-width="0.3" stroke-color="#000000"
%	 fill-color="#000000" fill-style="solid"
%	 />
%<ellipse p1="(26.88,20.62)" p2="(30.62,20.62)" p3="(30.62,16.88)" angle-start="0" angle-end="0" closure="open"
%	 stroke-width="0.3" stroke-color="#000000"
%	 fill-color="#000000" fill-style="solid"
%	 />
%<ellipse p1="(1.88,25.62)" p2="(5.62,25.62)" p3="(5.62,21.88)" angle-start="0" angle-end="0" closure="open"
%	 stroke-width="0.3" stroke-color="#000000"
%	 fill-color="#000000" fill-style="solid"
%	 />
%<ellipse p1="(1.88,15.62)" p2="(5.62,15.62)" p3="(5.62,11.88)" angle-start="0" angle-end="0" closure="open"
%	 stroke-width="0.3" stroke-color="#000000"
%	 fill-color="#000000" fill-style="solid"
%	 />
%<ellipse p1="(11.88,5.62)" p2="(15.62,5.62)" p3="(15.62,1.88)" angle-start="0" angle-end="0" closure="open"
%	 stroke-width="0.3" stroke-color="#000000"
%	 fill-color="#000000" fill-style="solid"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
\unitlength 1mm
\begin{picture}(30.62,35.62)(0,0)
\linethickness{0.3mm}
\multiput(3.75,23.75)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(3.75,13.75){\line(0,1){10}}
\linethickness{0.3mm}
\multiput(3.75,13.75)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(13.75,3.75)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(13.75,33.75)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(15.6,33.51){\line(0,1){0.49}}
\multiput(15.48,33.03)(0.13,0.47){1}{\line(0,1){0.47}}
\multiput(15.23,32.61)(0.12,0.21){2}{\line(0,1){0.21}}
\multiput(14.89,32.27)(0.12,0.12){3}{\line(0,1){0.12}}
\multiput(14.47,32.02)(0.21,0.12){2}{\line(1,0){0.21}}
\multiput(13.99,31.9)(0.47,0.13){1}{\line(1,0){0.47}}
\put(13.51,31.9){\line(1,0){0.49}}
\multiput(13.03,32.02)(0.47,-0.13){1}{\line(1,0){0.47}}
\multiput(12.61,32.27)(0.21,-0.12){2}{\line(1,0){0.21}}
\multiput(12.27,32.61)(0.12,-0.12){3}{\line(0,-1){0.12}}
\multiput(12.02,33.03)(0.12,-0.21){2}{\line(0,-1){0.21}}
\multiput(11.9,33.51)(0.13,-0.47){1}{\line(0,-1){0.47}}
\put(11.9,33.51){\line(0,1){0.49}}
\multiput(11.9,33.99)(0.13,0.47){1}{\line(0,1){0.47}}
\multiput(12.02,34.47)(0.12,0.21){2}{\line(0,1){0.21}}
\multiput(12.27,34.89)(0.12,0.12){3}{\line(0,1){0.12}}
\multiput(12.61,35.23)(0.21,0.12){2}{\line(1,0){0.21}}
\multiput(13.03,35.48)(0.47,0.13){1}{\line(1,0){0.47}}
\put(13.51,35.6){\line(1,0){0.49}}
\multiput(13.99,35.6)(0.47,-0.13){1}{\line(1,0){0.47}}
\multiput(14.47,35.48)(0.21,-0.12){2}{\line(1,0){0.21}}
\multiput(14.89,35.23)(0.12,-0.12){3}{\line(0,-1){0.12}}
\multiput(15.23,34.89)(0.12,-0.21){2}{\line(0,-1){0.21}}
\multiput(15.48,34.47)(0.13,-0.47){1}{\line(0,-1){0.47}}

\linethickness{0.3mm}
\put(30.6,18.51){\line(0,1){0.49}}
\multiput(30.48,18.03)(0.13,0.47){1}{\line(0,1){0.47}}
\multiput(30.23,17.61)(0.12,0.21){2}{\line(0,1){0.21}}
\multiput(29.89,17.27)(0.12,0.12){3}{\line(1,0){0.12}}
\multiput(29.47,17.02)(0.21,0.12){2}{\line(1,0){0.21}}
\multiput(28.99,16.9)(0.47,0.13){1}{\line(1,0){0.47}}
\put(28.51,16.9){\line(1,0){0.49}}
\multiput(28.03,17.02)(0.47,-0.13){1}{\line(1,0){0.47}}
\multiput(27.61,17.27)(0.21,-0.12){2}{\line(1,0){0.21}}
\multiput(27.27,17.61)(0.12,-0.12){3}{\line(1,0){0.12}}
\multiput(27.02,18.03)(0.12,-0.21){2}{\line(0,-1){0.21}}
\multiput(26.9,18.51)(0.13,-0.47){1}{\line(0,-1){0.47}}
\put(26.9,18.51){\line(0,1){0.49}}
\multiput(26.9,18.99)(0.13,0.47){1}{\line(0,1){0.47}}
\multiput(27.02,19.47)(0.12,0.21){2}{\line(0,1){0.21}}
\multiput(27.27,19.89)(0.12,0.12){3}{\line(1,0){0.12}}
\multiput(27.61,20.23)(0.21,0.12){2}{\line(1,0){0.21}}
\multiput(28.03,20.48)(0.47,0.13){1}{\line(1,0){0.47}}
\put(28.51,20.6){\line(1,0){0.49}}
\multiput(28.99,20.6)(0.47,-0.13){1}{\line(1,0){0.47}}
\multiput(29.47,20.48)(0.21,-0.12){2}{\line(1,0){0.21}}
\multiput(29.89,20.23)(0.12,-0.12){3}{\line(1,0){0.12}}
\multiput(30.23,19.89)(0.12,-0.21){2}{\line(0,-1){0.21}}
\multiput(30.48,19.47)(0.13,-0.47){1}{\line(0,-1){0.47}}

\linethickness{0.3mm}
\put(5.6,23.51){\line(0,1){0.49}}
\multiput(5.48,23.03)(0.13,0.47){1}{\line(0,1){0.47}}
\multiput(5.23,22.61)(0.12,0.21){2}{\line(0,1){0.21}}
\multiput(4.89,22.27)(0.12,0.12){3}{\line(0,1){0.12}}
\multiput(4.47,22.02)(0.21,0.12){2}{\line(1,0){0.21}}
\multiput(3.99,21.9)(0.47,0.13){1}{\line(1,0){0.47}}
\put(3.51,21.9){\line(1,0){0.49}}
\multiput(3.03,22.02)(0.47,-0.13){1}{\line(1,0){0.47}}
\multiput(2.61,22.27)(0.21,-0.12){2}{\line(1,0){0.21}}
\multiput(2.27,22.61)(0.12,-0.12){3}{\line(0,-1){0.12}}
\multiput(2.02,23.03)(0.12,-0.21){2}{\line(0,-1){0.21}}
\multiput(1.9,23.51)(0.13,-0.47){1}{\line(0,-1){0.47}}
\put(1.9,23.51){\line(0,1){0.49}}
\multiput(1.9,23.99)(0.13,0.47){1}{\line(0,1){0.47}}
\multiput(2.02,24.47)(0.12,0.21){2}{\line(0,1){0.21}}
\multiput(2.27,24.89)(0.12,0.12){3}{\line(0,1){0.12}}
\multiput(2.61,25.23)(0.21,0.12){2}{\line(1,0){0.21}}
\multiput(3.03,25.48)(0.47,0.13){1}{\line(1,0){0.47}}
\put(3.51,25.6){\line(1,0){0.49}}
\multiput(3.99,25.6)(0.47,-0.13){1}{\line(1,0){0.47}}
\multiput(4.47,25.48)(0.21,-0.12){2}{\line(1,0){0.21}}
\multiput(4.89,25.23)(0.12,-0.12){3}{\line(0,-1){0.12}}
\multiput(5.23,24.89)(0.12,-0.21){2}{\line(0,-1){0.21}}
\multiput(5.48,24.47)(0.13,-0.47){1}{\line(0,-1){0.47}}

\linethickness{0.3mm}
\put(5.6,13.51){\line(0,1){0.49}}
\multiput(5.48,13.03)(0.13,0.47){1}{\line(0,1){0.47}}
\multiput(5.23,12.61)(0.12,0.21){2}{\line(0,1){0.21}}
\multiput(4.89,12.27)(0.12,0.12){3}{\line(1,0){0.12}}
\multiput(4.47,12.02)(0.21,0.12){2}{\line(1,0){0.21}}
\multiput(3.99,11.9)(0.47,0.13){1}{\line(1,0){0.47}}
\put(3.51,11.9){\line(1,0){0.49}}
\multiput(3.03,12.02)(0.47,-0.13){1}{\line(1,0){0.47}}
\multiput(2.61,12.27)(0.21,-0.12){2}{\line(1,0){0.21}}
\multiput(2.27,12.61)(0.12,-0.12){3}{\line(0,-1){0.12}}
\multiput(2.02,13.03)(0.12,-0.21){2}{\line(0,-1){0.21}}
\multiput(1.9,13.51)(0.13,-0.47){1}{\line(0,-1){0.47}}
\put(1.9,13.51){\line(0,1){0.49}}
\multiput(1.9,13.99)(0.13,0.47){1}{\line(0,1){0.47}}
\multiput(2.02,14.47)(0.12,0.21){2}{\line(0,1){0.21}}
\multiput(2.27,14.89)(0.12,0.12){3}{\line(0,1){0.12}}
\multiput(2.61,15.23)(0.21,0.12){2}{\line(1,0){0.21}}
\multiput(3.03,15.48)(0.47,0.13){1}{\line(1,0){0.47}}
\put(3.51,15.6){\line(1,0){0.49}}
\multiput(3.99,15.6)(0.47,-0.13){1}{\line(1,0){0.47}}
\multiput(4.47,15.48)(0.21,-0.12){2}{\line(1,0){0.21}}
\multiput(4.89,15.23)(0.12,-0.12){3}{\line(1,0){0.12}}
\multiput(5.23,14.89)(0.12,-0.21){2}{\line(0,-1){0.21}}
\multiput(5.48,14.47)(0.13,-0.47){1}{\line(0,-1){0.47}}

\linethickness{0.3mm}
\put(15.6,3.51){\line(0,1){0.49}}
\multiput(15.48,3.03)(0.13,0.47){1}{\line(0,1){0.47}}
\multiput(15.23,2.61)(0.12,0.21){2}{\line(0,1){0.21}}
\multiput(14.89,2.27)(0.12,0.12){3}{\line(0,1){0.12}}
\multiput(14.47,2.02)(0.21,0.12){2}{\line(1,0){0.21}}
\multiput(13.99,1.9)(0.47,0.13){1}{\line(1,0){0.47}}
\put(13.51,1.9){\line(1,0){0.49}}
\multiput(13.03,2.02)(0.47,-0.13){1}{\line(1,0){0.47}}
\multiput(12.61,2.27)(0.21,-0.12){2}{\line(1,0){0.21}}
\multiput(12.27,2.61)(0.12,-0.12){3}{\line(0,-1){0.12}}
\multiput(12.02,3.03)(0.12,-0.21){2}{\line(0,-1){0.21}}
\multiput(11.9,3.51)(0.13,-0.47){1}{\line(0,-1){0.47}}
\put(11.9,3.51){\line(0,1){0.49}}
\multiput(11.9,3.99)(0.13,0.47){1}{\line(0,1){0.47}}
\multiput(12.02,4.47)(0.12,0.21){2}{\line(0,1){0.21}}
\multiput(12.27,4.89)(0.12,0.12){3}{\line(0,1){0.12}}
\multiput(12.61,5.23)(0.21,0.12){2}{\line(1,0){0.21}}
\multiput(13.03,5.48)(0.47,0.13){1}{\line(1,0){0.47}}
\put(13.51,5.6){\line(1,0){0.49}}
\multiput(13.99,5.6)(0.47,-0.13){1}{\line(1,0){0.47}}
\multiput(14.47,5.48)(0.21,-0.12){2}{\line(1,0){0.21}}
\multiput(14.89,5.23)(0.12,-0.12){3}{\line(1,0){0.12}}
\multiput(15.23,4.89)(0.12,-0.21){2}{\line(0,-1){0.21}}
\multiput(15.48,4.47)(0.13,-0.47){1}{\line(0,-1){0.47}}

\end{picture}


==> plsa.tex <==
%Created by jPicEdt 1.x
%Standard LaTeX format (emulated lines)
%Fri Jun 16 12:05:51 BST 2006
\unitlength 1mm
\begin{picture}(75.00,30.00)(0,0)

\linethickness{0.15mm}
%Ellipse 0 0(37.50,7.50)(15.00)(15.00)  arcStart=0.0 arcExtent=0.0
\put(44.98,7.01){\line(0,1){0.98}}
\multiput(44.86,8.96)(0.13,-0.97){1}{\line(0,-1){0.97}}
\multiput(44.60,9.91)(0.13,-0.47){2}{\line(0,-1){0.47}}
\multiput(44.23,10.82)(0.13,-0.30){3}{\line(0,-1){0.30}}
\multiput(43.74,11.67)(0.12,-0.21){4}{\line(0,-1){0.21}}
\multiput(43.14,12.45)(0.12,-0.16){5}{\line(0,-1){0.16}}
\multiput(42.45,13.14)(0.12,-0.12){6}{\line(1,0){0.12}}
\multiput(41.67,13.74)(0.16,-0.12){5}{\line(1,0){0.16}}
\multiput(40.82,14.23)(0.21,-0.12){4}{\line(1,0){0.21}}
\multiput(39.91,14.60)(0.30,-0.13){3}{\line(1,0){0.30}}
\multiput(38.96,14.86)(0.47,-0.13){2}{\line(1,0){0.47}}
\multiput(37.99,14.98)(0.97,-0.13){1}{\line(1,0){0.97}}
\put(37.01,14.98){\line(1,0){0.98}}
\multiput(36.04,14.86)(0.97,0.13){1}{\line(1,0){0.97}}
\multiput(35.09,14.60)(0.47,0.13){2}{\line(1,0){0.47}}
\multiput(34.18,14.23)(0.30,0.13){3}{\line(1,0){0.30}}
\multiput(33.33,13.74)(0.21,0.12){4}{\line(1,0){0.21}}
\multiput(32.55,13.14)(0.16,0.12){5}{\line(1,0){0.16}}
\multiput(31.86,12.45)(0.12,0.12){6}{\line(1,0){0.12}}
\multiput(31.26,11.67)(0.12,0.16){5}{\line(0,1){0.16}}
\multiput(30.77,10.82)(0.12,0.21){4}{\line(0,1){0.21}}
\multiput(30.40,9.91)(0.13,0.30){3}{\line(0,1){0.30}}
\multiput(30.14,8.96)(0.13,0.47){2}{\line(0,1){0.47}}
\multiput(30.02,7.99)(0.13,0.97){1}{\line(0,1){0.97}}
\put(30.02,7.01){\line(0,1){0.98}}
\multiput(30.02,7.01)(0.13,-0.97){1}{\line(0,-1){0.97}}
\multiput(30.14,6.04)(0.13,-0.47){2}{\line(0,-1){0.47}}
\multiput(30.40,5.09)(0.13,-0.30){3}{\line(0,-1){0.30}}
\multiput(30.77,4.18)(0.12,-0.21){4}{\line(0,-1){0.21}}
\multiput(31.26,3.33)(0.12,-0.16){5}{\line(0,-1){0.16}}
\multiput(31.86,2.55)(0.12,-0.12){6}{\line(0,-1){0.12}}
\multiput(32.55,1.86)(0.16,-0.12){5}{\line(1,0){0.16}}
\multiput(33.33,1.26)(0.21,-0.12){4}{\line(1,0){0.21}}
\multiput(34.18,0.77)(0.30,-0.13){3}{\line(1,0){0.30}}
\multiput(35.09,0.40)(0.47,-0.13){2}{\line(1,0){0.47}}
\multiput(36.04,0.14)(0.97,-0.13){1}{\line(1,0){0.97}}
\put(37.01,0.02){\line(1,0){0.98}}
\multiput(37.99,0.02)(0.97,0.13){1}{\line(1,0){0.97}}
\multiput(38.96,0.14)(0.47,0.13){2}{\line(1,0){0.47}}
\multiput(39.91,0.40)(0.30,0.13){3}{\line(1,0){0.30}}
\multiput(40.82,0.77)(0.21,0.12){4}{\line(1,0){0.21}}
\multiput(41.67,1.26)(0.16,0.12){5}{\line(1,0){0.16}}
\multiput(42.45,1.86)(0.12,0.12){6}{\line(1,0){0.12}}
\multiput(43.14,2.55)(0.12,0.16){5}{\line(0,1){0.16}}
\multiput(43.74,3.33)(0.12,0.21){4}{\line(0,1){0.21}}
\multiput(44.23,4.18)(0.13,0.30){3}{\line(0,1){0.30}}
\multiput(44.60,5.09)(0.13,0.47){2}{\line(0,1){0.47}}
\multiput(44.86,6.04)(0.13,0.97){1}{\line(0,1){0.97}}
%End Ellipse

\linethickness{0.15mm}
%Ellipse 0 0(67.50,7.50)(15.00)(15.00)  arcStart=0.0 arcExtent=0.0
\put(74.98,7.01){\line(0,1){0.98}}
\multiput(74.86,8.96)(0.13,-0.97){1}{\line(0,-1){0.97}}
\multiput(74.60,9.91)(0.13,-0.47){2}{\line(0,-1){0.47}}
\multiput(74.23,10.82)(0.13,-0.30){3}{\line(0,-1){0.30}}
\multiput(73.74,11.67)(0.12,-0.21){4}{\line(0,-1){0.21}}
\multiput(73.14,12.45)(0.12,-0.16){5}{\line(0,-1){0.16}}
\multiput(72.45,13.14)(0.12,-0.12){6}{\line(0,-1){0.12}}
\multiput(71.67,13.74)(0.16,-0.12){5}{\line(1,0){0.16}}
\multiput(70.82,14.23)(0.21,-0.12){4}{\line(1,0){0.21}}
\multiput(69.91,14.60)(0.30,-0.13){3}{\line(1,0){0.30}}
\multiput(68.96,14.86)(0.47,-0.13){2}{\line(1,0){0.47}}
\multiput(67.99,14.98)(0.97,-0.13){1}{\line(1,0){0.97}}
\put(67.01,14.98){\line(1,0){0.98}}
\multiput(66.04,14.86)(0.97,0.13){1}{\line(1,0){0.97}}
\multiput(65.09,14.60)(0.47,0.13){2}{\line(1,0){0.47}}
\multiput(64.18,14.23)(0.30,0.13){3}{\line(1,0){0.30}}
\multiput(63.33,13.74)(0.21,0.12){4}{\line(1,0){0.21}}
\multiput(62.55,13.14)(0.16,0.12){5}{\line(1,0){0.16}}
\multiput(61.86,12.45)(0.12,0.12){6}{\line(1,0){0.12}}
\multiput(61.26,11.67)(0.12,0.16){5}{\line(0,1){0.16}}
\multiput(60.77,10.82)(0.12,0.21){4}{\line(0,1){0.21}}
\multiput(60.40,9.91)(0.13,0.30){3}{\line(0,1){0.30}}
\multiput(60.14,8.96)(0.13,0.47){2}{\line(0,1){0.47}}
\multiput(60.02,7.99)(0.13,0.97){1}{\line(0,1){0.97}}
\put(60.02,7.01){\line(0,1){0.98}}
\multiput(60.02,7.01)(0.13,-0.97){1}{\line(0,-1){0.97}}
\multiput(60.14,6.04)(0.13,-0.47){2}{\line(0,-1){0.47}}
\multiput(60.40,5.09)(0.13,-0.30){3}{\line(0,-1){0.30}}
\multiput(60.77,4.18)(0.12,-0.21){4}{\line(0,-1){0.21}}
\multiput(61.26,3.33)(0.12,-0.16){5}{\line(0,-1){0.16}}
\multiput(61.86,2.55)(0.12,-0.12){6}{\line(0,-1){0.12}}
\multiput(62.55,1.86)(0.16,-0.12){5}{\line(1,0){0.16}}
\multiput(63.33,1.26)(0.21,-0.12){4}{\line(1,0){0.21}}
\multiput(64.18,0.77)(0.30,-0.13){3}{\line(1,0){0.30}}
\multiput(65.09,0.40)(0.47,-0.13){2}{\line(1,0){0.47}}
\multiput(66.04,0.14)(0.97,-0.13){1}{\line(1,0){0.97}}
\put(67.01,0.02){\line(1,0){0.98}}
\multiput(67.99,0.02)(0.97,0.13){1}{\line(1,0){0.97}}
\multiput(68.96,0.14)(0.47,0.13){2}{\line(1,0){0.47}}
\multiput(69.91,0.40)(0.30,0.13){3}{\line(1,0){0.30}}
\multiput(70.82,0.77)(0.21,0.12){4}{\line(1,0){0.21}}
\multiput(71.67,1.26)(0.16,0.12){5}{\line(1,0){0.16}}
\multiput(72.45,1.86)(0.12,0.12){6}{\line(0,1){0.12}}
\multiput(73.14,2.55)(0.12,0.16){5}{\line(0,1){0.16}}
\multiput(73.74,3.33)(0.12,0.21){4}{\line(0,1){0.21}}
\multiput(74.23,4.18)(0.13,0.30){3}{\line(0,1){0.30}}
\multiput(74.60,5.09)(0.13,0.47){2}{\line(0,1){0.47}}
\multiput(74.86,6.04)(0.13,0.97){1}{\line(0,1){0.97}}
%End Ellipse

\linethickness{0.15mm}
%Ellipse 0 0(7.50,7.50)(15.00)(15.00)  arcStart=0.0 arcExtent=0.0
\put(14.98,7.01){\line(0,1){0.98}}
\multiput(14.86,8.96)(0.13,-0.97){1}{\line(0,-1){0.97}}
\multiput(14.60,9.91)(0.13,-0.47){2}{\line(0,-1){0.47}}
\multiput(14.23,10.82)(0.13,-0.30){3}{\line(0,-1){0.30}}
\multiput(13.74,11.67)(0.12,-0.21){4}{\line(0,-1){0.21}}
\multiput(13.14,12.45)(0.12,-0.16){5}{\line(0,-1){0.16}}
\multiput(12.45,13.14)(0.12,-0.12){6}{\line(1,0){0.12}}
\multiput(11.67,13.74)(0.16,-0.12){5}{\line(1,0){0.16}}
\multiput(10.82,14.23)(0.21,-0.12){4}{\line(1,0){0.21}}
\multiput(9.91,14.60)(0.30,-0.13){3}{\line(1,0){0.30}}
\multiput(8.96,14.86)(0.47,-0.13){2}{\line(1,0){0.47}}
\multiput(7.99,14.98)(0.97,-0.13){1}{\line(1,0){0.97}}
\put(7.01,14.98){\line(1,0){0.98}}
\multiput(6.04,14.86)(0.97,0.13){1}{\line(1,0){0.97}}
\multiput(5.09,14.60)(0.47,0.13){2}{\line(1,0){0.47}}
\multiput(4.18,14.23)(0.30,0.13){3}{\line(1,0){0.30}}
\multiput(3.33,13.74)(0.21,0.12){4}{\line(1,0){0.21}}
\multiput(2.55,13.14)(0.16,0.12){5}{\line(1,0){0.16}}
\multiput(1.86,12.45)(0.12,0.12){6}{\line(1,0){0.12}}
\multiput(1.26,11.67)(0.12,0.16){5}{\line(0,1){0.16}}
\multiput(0.77,10.82)(0.12,0.21){4}{\line(0,1){0.21}}
\multiput(0.40,9.91)(0.13,0.30){3}{\line(0,1){0.30}}
\multiput(0.14,8.96)(0.13,0.47){2}{\line(0,1){0.47}}
\multiput(0.02,7.99)(0.13,0.97){1}{\line(0,1){0.97}}
\put(0.02,7.01){\line(0,1){0.98}}
\multiput(0.02,7.01)(0.13,-0.97){1}{\line(0,-1){0.97}}
\multiput(0.14,6.04)(0.13,-0.47){2}{\line(0,-1){0.47}}
\multiput(0.40,5.09)(0.13,-0.30){3}{\line(0,-1){0.30}}
\multiput(0.77,4.18)(0.12,-0.21){4}{\line(0,-1){0.21}}
\multiput(1.26,3.33)(0.12,-0.16){5}{\line(0,-1){0.16}}
\multiput(1.86,2.55)(0.12,-0.12){6}{\line(0,-1){0.12}}
\multiput(2.55,1.86)(0.16,-0.12){5}{\line(1,0){0.16}}
\multiput(3.33,1.26)(0.21,-0.12){4}{\line(1,0){0.21}}
\multiput(4.18,0.77)(0.30,-0.13){3}{\line(1,0){0.30}}
\multiput(5.09,0.40)(0.47,-0.13){2}{\line(1,0){0.47}}
\multiput(6.04,0.14)(0.97,-0.13){1}{\line(1,0){0.97}}
\put(7.01,0.02){\line(1,0){0.98}}
\multiput(7.99,0.02)(0.97,0.13){1}{\line(1,0){0.97}}
\multiput(8.96,0.14)(0.47,0.13){2}{\line(1,0){0.47}}
\multiput(9.91,0.40)(0.30,0.13){3}{\line(1,0){0.30}}
\multiput(10.82,0.77)(0.21,0.12){4}{\line(1,0){0.21}}
\multiput(11.67,1.26)(0.16,0.12){5}{\line(1,0){0.16}}
\multiput(12.45,1.86)(0.12,0.12){6}{\line(1,0){0.12}}
\multiput(13.14,2.55)(0.12,0.16){5}{\line(0,1){0.16}}
\multiput(13.74,3.33)(0.12,0.21){4}{\line(0,1){0.21}}
\multiput(14.23,4.18)(0.13,0.30){3}{\line(0,1){0.30}}
\multiput(14.60,5.09)(0.13,0.47){2}{\line(0,1){0.47}}
\multiput(14.86,6.04)(0.13,0.97){1}{\line(0,1){0.97}}
%End Ellipse

\linethickness{0.15mm}
%Polygon 0 1(45.00,7.50)(60.00,7.50) 
\put(45.00,7.50){\line(1,0){15.00}}
\put(60.00,7.50){\vector(1,0){0.12}}
%End Polygon

\linethickness{0.15mm}
%Polygon 0 1(30.00,7.50)(15.00,7.50) 
\put(15.00,7.50){\line(1,0){15.00}}
\put(15.00,7.50){\vector(-1,0){0.12}}
%End Polygon

\linethickness{0.15mm}
%Polygon 0 1(37.50,30.00)(37.50,15.00) 
\put(37.50,15.00){\line(0,1){15.00}}
\put(37.50,15.00){\vector(0,-1){0.12}}
%End Polygon

\put(67.50,7.50){\makebox(0,0)[cc]{$d$}}

\put(7.50,7.50){\makebox(0,0)[cc]{$w$}}

\put(37.50,7.50){\makebox(0,0)[cc]{$z$}}

\put(41.25,22.50){\makebox(0,0)[cc]{$P(z)$}}

\put(52.50,11.25){\makebox(0,0)[cc]{$P(d|z)$}}

\put(22.50,11.25){\makebox(0,0)[cc]{$P(w|z)$}}

\end{picture}

